Composing Neural Learning and Symbolic Reasoning with an Application to Visual Discrimination

We consider the problem of combining machine learning models to perform higher-level cognitive tasks with clear specifications. We propose the novel problem of Visual Discrimination Puzzles (VDP) that requires finding interpretable discriminators that classify images according to a logical specification. Humans can solve these puzzles with ease and they give robust, verifiable, and interpretable discriminators as answers. We propose a compositional neurosymbolic framework that combines a neural network to detect objects and relationships with a symbolic learner that finds interpretable discriminators. We create large classes of VDP datasets involving natural and artificial images and show that our neurosymbolic framework performs favorably compared to several purely neural approaches.

==> small-nobias-table.tex <==
\begin{table}[ht]
  %\centering
  \footnotesize
%   \hspace*{-1cm}
  \begin{tabular}{lll}
    \toprule
    {\bf Target Concept} & {\bf Sample Discriminators} & {\bf Natural
                                                         Language Reading}
     \\
    \midrule
    % (2on1 10, 3.json)

    % Two cats on a couch & $\exists x.~\forall y. \mathsf{cat}(x) \vee
    %                     \mathsf{right}(y,x)$ & \makecell[l]{``There is a
    %                                            cat or some thing \\ that all things are
    %                                            to the right of''} \\

    % \midrule

    % (allcatsonsofas 10, 21.json) & $\forall x.~\exists y. \mathsf{right}(x,y) \vee \mathsf{within}(x,y)$   \\
    % (allcatsonsofas 12, 21.json)
    % All cats are on sofas & $\exists x.~\forall
    %                                y. \mathsf{within}(y,x) \vee \neg
    %                                \mathsf{cat}(y)$  & ``There is
    %                                                    something that
    %                                                    all cats are within'' \\

    % (allcatsonsofas 15, 18.json)
                         % & $\forall x.~\forall
                         %   y. \mathsf{sofa}(x) \vee \neg
                         %   \mathsf{within}(y,x)$  &
                         %                            \makecell[l]{``Everything is either a sofa or it \\ does not have anything inside it''} \\

     % (allcatsonsofas 16, 18.json) & $\exists x.~\forall
     %                                  y. \mathsf{right}(y,x) \vee \mathsf{sofa}(x)$  \\

    % (allcatsonsofas 3, 18.json)
    %                      & $\exists x.~\exists
    %                                 y. \mathsf{sofa}(x) \wedge \mathsf{within}(y,x)$
    % & ``There is something on some sofa'' \\

     % (allcatsonsofas 5, 25.json)
    %                      & $\exists x.~\forall
    %                                 y. \mathsf{sofa}(y) \vee \mathsf{within}(y,x)$
    % & \makecell[l]{``There is something that has \\ every non-sofa within it''} \\

     % (allcatsonsofas 8, 18.json)
    All cats are on sofas & $\forall x.~\exists
                            y. \neg \mathsf{chair}(x) \wedge \neg \mathsf{sofa}(y)$
                                                      & ``There is no chair and there is some non-sofa'' \\

     % (allcatsonsofas 9, 18.json)
    %                      & $\exists x.~\exists
    %                                 y. \mathsf{cellphone}(y) \vee \mathsf{sofa}(x)$
    % & ``There is a cellphone or a sofa'' \\

    \midrule

    % (alldogsonsofas 1, 30.json)
    % All dogs are on sofas & $\forall x.~\forall
    %                               y. \neg\mathsf{bowl}(y)
    %                               \wedge \neg\mathsf{vase}(x)$
    %                                                    & ``There are
    %                                                      no bowls and
    %                                                      no vases''  \\

    % (alldogsonsofas 10, 32.json)
                         % & $\exists x.~\forall
                         %                y. \neg\mathsf{within}(y,x)
                         %                \vee \neg\mathsf{dog}(y)$  &
                         %                                             ``There
                         %                                             is
                         %                                             something that has every dog within it'' \\

    % (alldogsonsofas 11, 33.json)
    %                      & $\forall x.~\exists
    %                                y. \neg\mathsf{within}(x,y) \vee
    %                                \neg\mathsf{dog}(x)$  & ``For every dog
    % there is something it is within'' \\

    % (alldogsonsofas 3, 30.json)
    All dogs are on sofas & $\exists x.~\forall
                            y. \mathsf{within}(x,y) \vee
                            \neg\mathsf{sofa}(y)$  & ``There is
                                                     something that is within all sofas'' \\

    % (alldogsonsofas 8, 31.json)
                         % & $\exists x.~\exists
                         %          y. \mathsf{within}(y,x) \wedge
                         %          \neg\mathsf{dog}(y)$  & ``There is a
                         %                                  non-dog within something'' \\

    % \midrule
    % (catontv 1, 41.json)
    % Cat on TV & $\forall x.~\forall y. \mathsf{right}(x,y) \vee
    %             \neg\mathsf{within}(x,y)$ & \makecell[l]{``For every pair of
    %                                         things, either one is to
    %                                         the right \\ of the other or else
    %                                         it is not within the other''}  \\
    % (catontv 10, 50.json)
                         % & $\exists x.~\forall y. \mathsf{dog}(x) \vee
                         %   \mathsf{tvmonitor}(y)$ & ``Either there is
                         %                            a dog or everthing
                         %                            is a tv monitor'' \\
    % (catontv 11, 41.json) &  & $\exists x.~\exists y. \mathsf{dog}(y) \vee \mathsf{person}(x)$  &  \\
    % (catontv 13, 44.json) &  & $\exists x.~\forall y. \neg\mathsf{right}(x,y) \wedge \neg\mathsf{within}(y,x)$  &  \\
    % (catontv 14, 44.json) &  & $\forall x.~\forall y. \neg\mathsf{book}(x) \wedge \neg\mathsf{person}(y)$  &  \\
    % (catontv 15, 42.json) &  & $\exists x.~\exists y. \mathsf{cat}(x) \vee \mathsf{teddybear}(y)$  &  \\
    % (catontv 16, 43.json) &  & $\forall x.~\forall y. \mathsf{cat}(x) \vee \neg\mathsf{within}(x,y)$  &  \\
    % (catontv 17, 46.json) &  & $\forall x.~\forall y. \neg\mathsf{book}(y) \wedge \neg\mathsf{keyboard}(x)$  &  \\
    % (catontv 18, 46.json) &  & $\exists x.~\exists y. \mathsf{dog}(y) \vee \mathsf{person}(x)$  &  \\

    % (catontv 19, 46.json)
                         % & $\exists x.~\forall y. \mathsf{within}(x,y)
                         %   \vee \neg\mathsf{tvmonitor}(y)$  & ``There
                         %                                      is
                         %                                      something
                         %                                      within all tv monitors''\\
    % (catontv 2, 43.json) &  & $\exists x.~\forall y. \mathsf{dog}(x) \vee \mathsf{tvmonitor}(y)$  &  \\
    % (catontv 20, 42.json) &  & $\forall x.~\forall y. \neg\mathsf{right}(y,x) \vee \neg\mathsf{within}(y,x)$  &  \\
    % (catontv 3, 42.json) &  & $\forall x.~\forall y. \neg\mathsf{right}(y,x) \vee \neg\mathsf{tvmonitor}(y)$  &  \\
    % (catontv 7, 46.json) &  & $\forall x.~\forall y. \neg\mathsf{book}(x) \wedge \neg\mathsf{remote}(y)$  &  \\

    % \midrule
    % (desktop 20, 56.json) & $\forall x.~\forall y. \mathsf{left}(x,y) \vee \neg\mathsf{within}(x,y)$  & 18  \\
    % (desktop 7, 60.json)
    %                    Desktop computer  & $\forall x.~\forall
    %                                        y. \neg\mathsf{sofa}(x)
    %                                        \wedge
    %                                        \neg\mathsf{within}(x,y)$
    %                                                    & \makecell[l]{``There is no
    % sofa and \\ there is nothing within anything else''} \\

    % \midrule
    % (dogherded 16, 80.json)
    % Dog herding sheep & $\exists x.~\forall y. \mathsf{truck}(x) \vee
    %               \neg\mathsf{person}(y)$ & ``There is a truck or
    %                                         there is no person''\\
    % (dogherded 18, 77.json) &  & $\exists x.~\exists y. \mathsf{car}(y) \vee \mathsf{person}(x)$  &  \\
    % (dogherded 3, 82.json)
    % Dog herding sheep & $\forall x.~\exists y. \mathsf{right}(x,y)
    %                     \vee \neg\mathsf{sheep}(x)$ & \makecell[l]{``Every
    %                                                   sheep has
    %                                                   something \\ that
    % it is to the
    % right of''}  \\

    % \midrule
    % (drivingdirection 1, 6, 8; 219, 220, 219.json) &  & $\forall x.~\exists y. \mathsf{right}(x,y) \vee \mathsf{truck}(y)$  &  \\
    % (drivingdirection 11, 218.json) &  & $\exists x.~\forall y. \mathsf{right}(x,y) \vee \mathsf{truck}(x)$  &  \\
    % (drivingdirection 12, 2 ; 219, 219.json) &  & $\forall x.~\exists y. \mathsf{truck}(y) \vee \neg\mathsf{person}(x)$  &  \\
    % (drivingdirection 14, 4 ; 224, 225.json) &  & $\forall x.~\forall y. \neg\mathsf{pottedplant}(y) \wedge \neg\mathsf{umbrella}(x)$  &  \\
    % (drivingdirection 15, 18 ; 225, 224.json) &  & $\forall x.~\forall y. \neg\mathsf{clock}(x) \wedge \neg\mathsf{pottedplant}(y)$  &  \\

    % (drivingdirection 16, 9 ; 221, 221.json)
    % Driving direction & $\forall x.~\exists y. \mathsf{left}(y,x) \vee
    %                     \neg\mathsf{car}(x)$ & ``Every car has
    %                                            something to its left''  \\
    % (drivingdirection 17, 224.json) &  & $\exists x.~\exists y. \mathsf{within}(y,x) \vee \mathsf{within}(x,y)$  &  \\
    % (drivingdirection 19, 221.json) &  & $\exists x.~\forall y. \mathsf{car}(y) \vee \mathsf{truck}(x)$  &  \\
    % (drivingdirection 20, 222.json) &  & $\forall x.~\forall y. \neg\mathsf{backpack}(y) \wedge \neg\mathsf{umbrella}(x)$  &  \\
    % (drivingdirection 3, 222.json) &  & $\exists x.~\exists y. \mathsf{handbag}(x) \vee \mathsf{within}(x,y)$  &  \\
    % (drivingdirection 5, 224.json) &  & $\exists x.~\exists y. \mathsf{backpack}(x) \vee \mathsf{handbag}(y)$  &  \\
    % (drivingdirection 7, 220.json)
                         % & $\forall x.~\exists y. \mathsf{truck}(y)
                         %   \vee \neg\mathsf{car}(x)$ & ``There is a
                         %                               truck or there
                         %                               is no car''  \\

    \midrule
    % (kitchen 1, 95.json) & 20 & $\exists x.~\exists y. \mathsf{cup}(x) \vee \mathsf{within}(x,y)$  &   \\
    % (kitchen 10, 92.json) &  & $\forall x.~\forall y. \neg\mathsf{book}(x) \wedge \neg\mathsf{toilet}(y)$  &   \\
    % (kitchen 11, 93.json) &  & $\forall x.~\exists y. \neg\mathsf{chair}(x) \wedge \neg\mathsf{cup}(y)$  &   \\

    % (kitchen 17, 92.json)
    Kitchen & $\exists x.~\exists y. \mathsf{banana}(y) \vee
              \mathsf{oven}(x)$ & ``There is either a banana or an oven''   \\
    % (kitchen 19, 93.json) &  & $\forall x.~\forall y. \neg\mathsf{cup}(x) \vee \neg\mathsf{refrigerator}(y)$  &   \\
    % (kitchen 2, 7 ; 90, 90.json) &  & $\exists x.~\exists y. \mathsf{oven}(x) \vee \mathsf{toilet}(y)$  &   \\
    % (kitchen 20, 95.json) &  & $\exists x.~\exists y. \mathsf{bowl}(x) \vee \mathsf{within}(x,y)$  &   \\
    % (kitchen 4, 90.json) &  & $\exists x.~\forall y. \neg\mathsf{chair}(y) \wedge \neg\mathsf{right}(x,y)$  &   \\
    % (kitchen 5, 91.json) &  & $\forall x.~\exists y. \mathsf{oven}(y) \vee \neg\mathsf{cup}(x)$  &   \\
    % (kitchen 6, 92.json) &  & $\exists x.~\forall y. \mathsf{oven}(x) \vee \mathsf{right}(x,y)$  &   \\

    % (kitchen 8, 90.json)
                         % & $\forall x.~\exists y. \mathsf{left}(x,y)
                         %   \vee \neg\mathsf{cup}(x)$ & ``Every cup is
                         %                               to the left of something''  \\

    % \midrule
  %  (parkmeter 1, 10, 12, 17, 2, 7 ; 106, 106, 106, 106, 106, 106.json) & 20& $\exists x.~\forall
  %                                y. \mathsf{bus}(x) \vee \neg\mathsf{truck}(y)$   & 20  \\

    % (parkmeter 13, 6, 8 ; 105, 108, 104.json)
    % Parking meter in sight & $\forall x.~\exists y. \mathsf{left}(x,y)
    %                          \vee \mathsf{parkingmeter}(y)$ & \makecell[l]{``There
    %                                                           is a
    %                                                           parking
    %                                                           meter or
    %                                                           else \\ everything is to the left of something''} \\
  %  (parkmeter 20 ; 104.json) & & $\exists x.~\forall
  %                                y. \mathsf{left}(x,y) \vee \mathsf{parkingmeter}(x)$   &   \\
  %  (parkmeter 5 ; 104.json) & & $\forall x.~\exists
  %                                y. \mathsf{parkingmeter}(y) \vee \neg\mathsf{truck}(x)$   &   \\

    \midrule
  %  (personball 1, 14, 8 ; 117, 117, 114.json) & 20& $\exists x.~\exists y. \mathsf{bottle}(y) \vee \mathsf{within}(y,x)$  & 13  \\
  %  (personball 10, 12, 9 ; 117, 114, 114.json) & & $\forall x.~\forall y. \neg\mathsf{chair}(y) \wedge \neg\mathsf{dog}(x)$  &   \\
  %  (personball 11, 114.json) & & $\exists x.~\exists y. \mathsf{diningtable}(y) \vee \mathsf{within}(x,y)$  &   \\
  %  (personball 13, 17 ; 121, 116.json) & & $\forall x.~\forall y. \neg\mathsf{cup}(y) \wedge \neg\mathsf{elephant}(x)$  &   \\
  %  (personball 16, 6 ; 117, 114.json) & & $\forall x.~\forall y. \neg\mathsf{bench}(y) \wedge \neg\mathsf{dog}(x)$  &   \\
  %  (personball 18 ; 118.json) & & $\forall x.~\forall y. \neg\mathsf{bench}(y) \wedge \neg\mathsf{bottle}(x)$  &   \\

    % (personball 19 ; 119.json)
    People playing with ball & $\forall x.~\forall
                      y. \mathsf{person}(x) \vee
                      \neg\mathsf{had~by}(y,x)$ &
                                                  \makecell[l]{``Everything
                                                  is either a person \\ or else nothing has it''} \\
  %  (personball 2, 4 ; 115, 116.json) & & $\forall x.~\forall y. \neg\mathsf{diningtable}(y) \wedge \neg\mathsf{dog}(x)$  &   \\
  %  (personball 20 ; 114.json) & & $\forall x.~\forall y. \neg\mathsf{bench}(y) \wedge \neg\mathsf{elephant}(x)$  &   \\
  %  (personball 5 ; 119.json) & & $\forall x.~\forall y. \neg\mathsf{bench}(x) \wedge \neg\mathsf{cup}(y)$  &   \\
  %  (personball 7 ; 118.json) & & $\forall x.~\forall y. \neg\mathsf{bowl}(x) \wedge \neg\mathsf{chair}(y)$  &   \\

     % \midrule
    % (populatedbus 18 ; 130.json)
    % Bus with people inside & $\exists x.~\exists y. \mathsf{bus}(x)
    %                          \wedge \mathsf{right}(x,y)$ & ``There is
    %                                                        a bus to
    %                                                        the right
    %                                                        of something'' \\
    % (populatedbus 4 ; 130.json)
    % Bus with people in it & $\exists x.~\exists y. \neg\mathsf{bus}(x)
    %                          \wedge \neg\mathsf{within}(x,y)$ & \makecell[l]{``There
    %                                                             is a non-bus
    %                                                             and
    %                                                             something \\
    % that it is
    % not
    % within''} \\
  %  (populatedbus 5, 6 ; 130, 130.json) &  & $\exists x.~\forall y. \mathsf{backpack}(x) \vee \neg\mathsf{car}(y)$  &    \\

  % \midrule
  %  (pplandties 1, 13, 14, 20, 6, 9 ; 139, 139, 140, 139, 139, 140.json) & 20& $\exists x.~\forall y. \mathsf{right}(x,y) \vee \mathsf{tie}(x)$  & 20    \\

    % (pplandties 10, 145.json)
    % People and ties & $\forall x.~\exists
    %                   y. \mathsf{tie}(y) \vee
    %                   \mathsf{within}(x,y)$ &
    %                                           \makecell[l]{``There
    %                                           is
    %                                           a
    %                                           tie
    %                                           or else \\ everything is within something''} \\
  %  (pplandties 11, 19 ; 139, 139.json) & & $\forall x.~\exists y. \mathsf{right}(y,x) \vee \mathsf{tie}(y)$  &     \\
  %  (pplandties 12, 8 ; 140, 145.json) & & $\exists x.~\forall y. \mathsf{tie}(x) \vee \mathsf{within}(y,x)$  &     \\
  %  (pplandties 15, 16, 4, 7 ; 137, 142, 143, 143.json) & & $\exists x.~\exists y. \mathsf{bottle}(y) \vee \mathsf{within}(y,x)$  &     \\
  %  (pplandties 17, 140.json) & & $\forall x.~\exists y. \mathsf{person}(x) \vee \mathsf{right}(x,y)$  &     \\
  %  (pplandties 18, 5 ; 143, 143.json) & & $\exists x.~\exists y. \mathsf{within}(y,x) \vee \mathsf{within}(x,y)$  &     \\
  %  (pplandties 2, 3 ; 137, 137.json) & & $\exists x.~\exists y. \mathsf{fork}(x) \vee \mathsf{within}(y,x)$  &     \\

    % \midrule
  %  (pplwearingties 1, 20 ; 152, 152.json) & 20 & $\forall x.~\exists y. \mathsf{right}(x,y) \vee \mathsf{tie}(y)$  &     \\
  %  (pplwearingties 10, 15; 152, 152.json) &  & $\exists x.~\forall y. \mathsf{left}(y,x) \vee \mathsf{tie}(x)$  &     \\
  %  (pplwearingties 13, 3 ; 152, 152.json) &  & $\exists x.~\exists y. \mathsf{tie}(x) \wedge \mathsf{within}(x,y)$  &     \\
  %  (pplwearingties 19, 7 ; 152, 152.json) & 20 & $\forall x.~\exists y. \mathsf{person}(x) \vee \mathsf{right}(x,y)$  &     \\

    % (pplwearingties 2, 8 ; 152, 152.json)
    % People wearing ties & $\exists x.~\forall
    %                       y. \mathsf{right}(x,y) \vee
    %                       \mathsf{tie}(x)$ & \makecell[l]{``There is a tie or else
    %                                          there is \\ something to the
    % right of everything''} \\

    % (pplwearingties 4, 152.json) & 20 & $\exists x.~\exists y. \mathsf{right}(x,y) \wedge \mathsf{tie}(x)$  &     \\

    % \midrule
    % (sleeping 1 ; 177.json)
    % Someone sleeping on a bench & $\exists x.~\forall
    %                               y. \neg\mathsf{left}(y,x) \wedge
    %                               \neg\mathsf{within}(y,x)$ & \makecell[l]{``There
    %                                                           is
    %                                                           something
    %                                                           with
    %                                                           nothing
    %                                                           to the
    %                                                           left of
    %                                                           it \\ and nothing within it''} \\
  %  (sleeping 10 ; 173.json)  & & $\exists x.~\exists y. \mathsf{person}(x) \vee \mathsf{pottedplant}(y)$   &   \\
  %  (sleeping 11, 16, 3, 9 ; 174, 174, 174, 174.json)  & & $\exists x.~\forall y. \mathsf{person}(x) \vee \mathsf{right}(x,y)$   &   \\
  %  (sleeping 12, 13, 7 ; 171, 177, 171.json)  & & $\exists x.~\forall y. \mathsf{bench}(y) \vee \mathsf{right}(x,y)$   &   \\
  %  (sleeping 14, 6 ; 172, 172.json)  & & $\forall x. \mathsf{bench}(x) \vee \mathsf{person}(x)$   &   \\
  %  (sleeping 15 ; 173.json)  & & $\exists x.~\forall y. \mathsf{left}(x,y) \vee \mathsf{person}(x)$   &   \\
  %  (sleeping 17 ; 171.json)  & & $\exists x.~\forall y. \neg\mathsf{left}(y,x) \wedge \neg\mathsf{within}(y,x)$   &   \\
  %  (sleeping 18 ; 173.json)  & & $\exists x.~\forall y. \mathsf{person}(x) \vee \mathsf{within}(x,y)$   &   \\
  %  (sleeping 19 ; 175.json)  & & $\forall x.~\forall y. \neg\mathsf{left}(x,y) \vee \neg\mathsf{within}(x,y)$   &   \\
  %  (sleeping 2 ; 179.json)  & & $\forall x.~\exists y. \mathsf{person}(y) \vee \mathsf{within}(y,x)$   &   \\
  %  (sleeping 20 ; 177.json)  & & $\forall x.~\forall y. \mathsf{person}(y) \vee \neg\mathsf{within}(y,x)$   &   \\
  %  (sleeping 4 ; 172.json)  & & $\forall x.~\forall y. \mathsf{left}(y,x) \vee \neg\mathsf{within}(x,y)$   &   \\

  %  (sleeping 5 ; 171.json)
                         % & $\exists x.~\exists y. \mathsf{right}(y,x)
                         %   \wedge \neg\mathsf{bench}(x)$ & ``There is
                         %                                   something
                         %                                   to the
                         %                                   right of
                         %                                   a non-bench'' \\
  %  (sleeping 8 ; 175.json)  & & $\forall x.~\forall y. \neg\mathsf{cat}(x) \wedge \neg\mathsf{pottedplant}(y)$   &   \\

    % \midrule
  %  (umbrella 10, 16, 20, 3, 4 ; 209, 209, 209, 209, 209.json)  & 20& $\forall x.~\exists y. \mathsf{right}(x,y) \vee \mathsf{umbrella}(y)$   & 20  \\
  %  (umbrella 15, 18, 8 ; 208, 211, 208.json)  & & $\exists x.~\exists y. \mathsf{chair}(y) \vee \mathsf{handbag}(x)$   & \\

  %  (umbrella 2 ; 208.json)
    % Umbrella weather & $\exists x.~\forall y. \mathsf{umbrella}(x)
    %                    \vee \mathsf{within}(x,y)$ & \makecell[l]{``There is an
    %                                                 umbrella or else \\
    %                                                 there is something
    %                                                 within everything''} \\
  %  (umbrella 6 ; 211.json)  & & $\forall x.~\exists y. \mathsf{car}(y) \vee \neg\mathsf{person}(x)$   & \\

    \bottomrule
  \end{tabular}
      \caption{Sample discriminators found without the biases discussed
        in Section~\ref{symbolic}. }
      \label{nonguardedtable}
\end{table}

% \begin{table}
%     \begin{tabular}{lll}
%     Sample Table   & Column A  & Column B  \\
%     Sample Value   & 1.0       & 2.0       \\
%     Sample Value 2 & 2.0       & 3.0       \\
%     Sample Value 3 & \texttt{code here} & $\pi = 3.14$ \\
%     \end{tabular}
%     \label{nonguardedtable}
% \end{table}
